The Branching-Course MPC Algorithm for Maritime Collision Avoidance

This article presents a new algorithm for short-term maritime collision avoidance (COLAV) named the branching-course MPC (BC-MPC) algorithm. The algorithm is designed to be robust with respect to noise on obstacle estimates, which is a significant source of disturbance when using exteroceptive sensors such as e.g. radars for obstacle detection and tracking. Exteroceptive sensors do not require vessel-to-vessel communication, which enables COLAV toward vessels not equipped with e.g. automatic identification system (AIS) transponders, in addition to increasing the robustness with respect to faulty information which may be provided by other vessels. The BC-MPC algorithm is compliant with rules 8 and 17 of the International Regulations for Preventing Collisions at Sea (COLREGs), and favors maneuvers following rules 13-15. This results in a COLREGs-aware algorithm which can ignore rules 13-15 when necessary. The algorithm is experimentally validated in several full-scale experiments in the Trondheimsfjord in 2017 using a radar-based system for obstacle detection and tracking. The COLAV experiments show good performance in compliance with the desired algorithm behavior.

==> parts/bc-mpc_old.tex <==
%!TEX root=../root.tex
The \gls{bc-mpc} algorithm is intended to avoid collisions with moving obstacles while respecting dynamic constraints of the vessel in order to ensure feasible maneuvers, which is ideal for short-term \gls{colav}. The algorithm is based on \acrfull{mpc}, and plans vessel-feasible trajectories with multiple maneuvers where only the first maneuver is executed. The trajectories have continuous acceleration, which can be beneficial in vessel controllers utilizing acceleration feedforward. The algorithm is designed with robustness to noisy obstacle estimates in mind, to fit well with tracking systems based on exteroceptive sensors, for instance radars. Furthermore, the algorithm is modular, so the algorithm can easily be tailored for different applications.

The algorithm is designed with the short-term perspective of \gls{colregs} in mind. The algorithm can be described by two steps:
\begin{enumerate}
	\item Generate a search space consisting of trajectories feasible with respect to the dynamic constraints of the vessel
	\item Discretize the search space and compute an objective function value on the trajectories. The optimal trajectory is then selected as the one with the minimum objective function value.
\end{enumerate}

The \gls{bc-mpc} algorithm architecture is shown in \cref{fig:bc-mpc_architecture}. The algorithm inputs a desired trajectory, which can originate from either another \gls{colav} algorithm or directly from a user. The guidance function receives the desired trajectory, and computes a desired acceleration given a vessel state and time specified by the trajectory generation. The trajectory generation block creates a set of possible vessel trajectories, given an initial vessel state, initial desired velocity and desired accelerations from the guidance function. A tracking system provides obstacle estimates, which are used to calculate a part of the objective function. The optimization block computes the optimal trajectory based on the objective function \eqref{eq:objFunc} and outputs this as a desired velocity trajectory to the vessel controllers \eqref{eq:vesselController}.
\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/bc-mpc_architecture.pdf}
	\caption{\label{fig:bc-mpc_architecture}BC-MPC algorithm overview.}
\end{figure}

\subsection{Trajectory generation}
The search space consists of a number of trajectories, each with a sequence of maneuvers. This section describes how the trajectories are generated. Each trajectory is defined by a desired velocity trajectory containing a \gls{sog} and course trajectory with continuous acceleration, and a feedback-corrected position trajectory.

\subsubsection{Trajectory generation: A single step}
As mentioned, each trajectory consists of a sequence of maneuvers, resulting in trajectories that branches out from each other. Hence, the trajectory generation can be divided in repeatable steps. At each step, a set of sub-trajectories, each containing one maneuver, are computed given an initial vessel configuration, initial time and some step specific parameters:
\begin{itemize}
	\item The number of \gls{sog} maneuvers
	\item The number of course maneuvers
	\item The time allowed for changing the actuator input, named the ramp time
	\item The maneuver time length in \gls{sog} and course
	\item The total step time length
\end{itemize}

We start by generating the desired velocity trajectories, which all should be feasible with respect to actuator rate and magnitude saturations. To ensure feasibility with respect to the actuator rate saturations, we start from the model \eqref{eq:Model} by calculating the possible \gls{sog} and course accelerations given our current configuration as:
\begin{equation}\label{eq:possibleAcc}
	\begin{aligned}
		\dot{\bs X}_{\max} &= \bs M^{-1}\left( \bs\tau_{\max} - \bs\sigma(\bs X_0) \right) \\
		\dot{\bs X}_{\min} &= \bs M^{-1}\left( \bs\tau_{\min} - \bs\sigma(\bs X_0) \right),
	\end{aligned}
\end{equation}
where $\dot{\bs X}_{\max} = \begin{bmatrix} \dot U_{\max} & \dot r_{\max} \end{bmatrix}^T$, $\dot{\bs X}_{\min} = \begin{bmatrix} \dot U_{\min} & \dot r_{\min} \end{bmatrix}^T$, $\bs X_0$ is the current vessel velocity and:
\begin{equation}\label{eq:possibleActuator}
	\begin{aligned}
		\bs\tau_{\max} &= \text{sat}\left(\bs \tau_0 + T_{ramp} \dot{\bs \tau}_{\max}, \bs \tau_{\min},  \bs \tau_{\max}\right) \\
		\bs\tau_{\min} &= \text{sat}\left(\bs \tau_0 + T_{ramp} \dot{\bs \tau}_{\min}, \bs \tau_{\min},  \bs \tau_{\max}\right),
	\end{aligned}
\end{equation}
where $T_{ramp}$ is the ramp time, $\bs \tau_0$ is the current control input, $\bs \tau_{\max}$ and $\bs \tau_{\min}$ is the maximum and minimum control input, respectively, $\dot{\bs \tau}_{\max}$ and $\dot{\bs \tau}_{\min}$ is the maximum and minimum control input rate of change, respectively. The saturation function $\text{sat}(\bs a,\bs a_{\min},\bs a_{\max})$ is defined as $\text{sat}:\mathbb{R}^K\times\mathbb{R}^K\times\mathbb{R}^K \rightarrow \mathbb{R}^K$ with:
% \begin{equation}
% 	\text{sat}(\bs a,\bs a_{\min},\bs a_{\max}) = \min\left(\max\left( \bs a, \bs a_{\min}\right), \bs a_{\max} \right),
% \end{equation}
\begin{equation}
	a^*_i = \begin{cases} 
  	 a_{\min,i}     &, a_i < a_{\min,i} \\
  	 a_{\max,i}     &, a_i > a_{\max,i} \\
  	 a_i			&, \text{otherwise},
  	\end{cases}
\end{equation}
for $\bs a^* = \text{sat}(\bs a,\bs a_{\min},\bs a_{\max})$, $i\in\{1,2,\ldots,K\}$ and $(\cdot)_i$ being element $i$ of a vector. Following this, we create a set of possible accelerations as:
\begin{equation}
	A_d = \left\{ (\dot U, \dot r) \in \mathbb{R}\times\mathbb{R} \big | \dot U \in [\dot U_{\min}, \dot U_{\max}], \dot r \in [\dot r_{\min}, \dot r_{\max}] \right\}.
\end{equation}
The set of possible accelerations is then sampled uniformly to create a discrete set of candidate maneuver accelerations:
\begin{equation}
	\begin{aligned}
		\dot{\bs U}_{samples} &= \left\{ \dot U_{\max,1}, \dot U_{\max,2}, \ldots, \dot U_{\max,N_U} \right\} \\
		\dot{\bs r}_{samples} &= \left\{ \dot r_{\max,1}, \dot r_{\max,2}, \ldots, \dot r_{\max,N_\chi} \right\},
	\end{aligned}
\end{equation}
where $\dot U_{\max,1}$, $i\in [1,N_U]$ are $N_U$ \gls{sog} acceleration samples and $\dot r_{\max,1}$, $i\in [1,N_\chi]$ are $N_\chi$ course acceleration samples. To be able to include a specific maneuver in the search space, we allow to modify some of the sampled accelerations if a desired acceleration $(\dot U'_d, \dot r'_d)$ is inside the set of possible accelerations as follows: If $\dot U'_d \in A_d$, we change the closest \gls{sog} acceleration sample in $\dot{\bs U}_{samples}$ to $\dot U'_d$. Similarly for course, if $\dot r'_d \in A_d$, we change the closest course acceleration sample in $\dot{\bs r}_{samples}$ to $\dot r'_d$. Following this, we create a set of candidate maneuver accelerations by combining the \gls{sog} and course candidate maneuvers as $\dot{\bs U}_{samples} \times \dot{\bs r}_{samples}$. This concept is illustrated in \cref{fig:AccSamples}, where $A_d$ is sampled with $N_U = 3$ \gls{sog} samples and $N_\chi = 5$ course samples.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{figures/AccelerationSamples.pdf}
	\caption{\label{fig:AccSamples}Set of possible acceleration in blue, with initial samples shown as blue circles. The desired acceleration $(\dot U'_d, \dot r'_d)$ is shown as a green circle, while the modified samples is shown as red crosses.}
\end{figure}

Given the acceleration samples, we create a set of $N_U$ motion primitives for \gls{sog} based on the acceleration trajectories:
\begin{equation}\label{eq:sog_acc}
  	\dot U_{d,i}(t) = \begin{cases} 
  	 k_{U,i} t                                      &, 0 \leq t < T_{ramp}  \\
  	 \dot U_{i_{\max}}                              &, T_{ramp} \leq t < T_U - T_{ramp} \\
  	 \dot U_{i_{\max}} - k_{U,i} (t - (T_U - T_{ramp})) &, T_U - T_{ramp} \leq t < T_U \\
  	 0,                                             &, T_U \leq t \leq T,
  	\end{cases}
\end{equation}
where $k_{U,i} = \frac{\dot U_{\max,i}}{T_{ramp}}$, $\dot U_{\max,i}$ is the sampled acceleration for \gls{sog} motion primitive $i\in[1,N_U]$, $T_U$ is the \gls{sog} maneuver length and $T$ is the total trajectory length. Similarly, we define $N_\chi$ course motion primitives by the acceleration trajectories:
\begin{equation}\label{eq:course_acc}
  	\dot r_{d,i}(t) = \begin{cases} 
  	 k_{r,i} t                                        			&, 0 \leq t < T_{ramp}  \\
  	 2 \dot r_{i_{\max}} - k_{r,i} t                      		&, T_{ramp} \leq t < 2 T_{ramp} \\
  	 0                                                			&, 2 T_{ramp} \leq t < T_\chi - 2 T_{ramp} \\
  	 -k_{r,i} (t - (T_\chi - 2 T_{ramp}))                     	&, T_\chi - 2 T_{ramp} \leq t < T_\chi - T_{ramp}  \\
  	 -2 \dot r_{i_{\max}} + k_{r,i} (t - (T_\chi - T_{ramp})) 	&, T_\chi - T_{ramp} \leq t < T_\chi \\
  	 0                                                			&, 2 T_\chi \leq t < T,
  	\end{cases}
\end{equation}
where $k_{r,i} = \frac{\dot r_{\max,i}}{T_{ramp}}$, $\dot r_{\max,i}$ is the sampled acceleration for course motion primitive $i\in[1,N_\chi]$ and $T_\chi$ is the course maneuver length. The acceleration trajectories for $N_U = 3$ \gls{sog} motion primitives and $N_\chi = 5$ course motion primitives are illustrated in \cref{fig:motionPrimitives}. Notice that the integral of the course acceleration maneuvers are zero, hence if the maneuver is initialized with zero \gls{rot} the maneuver will end with zero \gls{rot}.
\begin{figure}
  	\centering
  	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/UdotTraj.pdf}
    	\caption{SOG acceleration motion primitives}
  	\end{subfigure} \\
  	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/rdotTraj.pdf}
    	\caption{Yaw acceleration motion primitives. Note that the integral of each acceleration trajectory is zero.}
  	\end{subfigure}
  	\caption{\label{fig:motionPrimitives}Acceleration motion primitives}
\end{figure}

Based on the acceleration trajectories, we create trajectories for the desired \gls{sog}, \gls{rot} and course by symbolically integrating the expressions \eqref{eq:sog_acc} and \eqref{eq:course_acc} as:
\begin{equation}\label{eq:velocity_trajs}
	\begin{aligned}
		U_{d,i}(t) &= U_{d,0} + \int_{t_0}^t \dot U_{d,i}(\gamma) \mathrm{d}\gamma, \quad i \in [1,N_U] \\
		r_{d,i}(t) &= r_{d,0} + \int_{t_0}^t \dot r_{d,i}(\gamma) \mathrm{d}\gamma, \quad i \in [1,N_\chi] \\
		\chi_{d,i}(t) &= \chi_{d,0} + \int_{t_0}^t r_{d,i}(\gamma) \mathrm{d}\gamma, \quad i \in [1,N_\chi]. \\
	\end{aligned}
\end{equation}
The initial values $U_{d,0}$, $r_{d,0}$ and $\chi_{d,0}$ are taken as the corresponding desired values from the last iteration (or step, if computing trajectories for a branch), such that the desired trajectories passed to the vessel controllers are continuous. Note that this implies that we do not include feedback in the desired trajectories. Furthermore, as in \cref{sec:ASVmodelingControl}, the vessel sideslip is neglected. This could, however, be included by using a vessel model including sideslip. A numerical example of $5$ \gls{sog} and $5$ course trajectories are shown in \cref{fig:SOGtraj,fig:Coursetraj}, where a maneuver length of $5~\si{\second}$ are used for both \gls{sog} and course. Rule 8 of \gls{colregs} requires that maneuvers are of such a magnitude that they appear as readily observable for other vessels. By selecting the initial yaw rate in \eqref{eq:velocity_trajs} as $r_{d,0} = 0$ we ensure that maneuvers start and end with constant-course motion, which produce maneuvers that should be readily observable for other vessels. 
\begin{figure}
	\centering
	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/traj_U_acc.pdf}
  	\end{subfigure} \\
	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/traj_U.pdf}
  	\end{subfigure}
  	%\includegraphics[width=.7\textwidth]{figures/sogTraj.png}
  	\caption{\gls{sog} trajectory. Acceleration in the top plot and speed in the bottom plot.\label{fig:SOGtraj}}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/traj_r_acc.pdf}
  	\end{subfigure} \\
	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/traj_r.pdf}
  	\end{subfigure} \\
  	\begin{subfigure}[b]{.7\textwidth}
    	\includegraphics[width=\textwidth]{figures/traj_psi.pdf}
  	\end{subfigure}
  	%\includegraphics[width=.7\textwidth]{figures/yawTraj.png}
  	\caption{Course trajectory. Acceleration in the top plot, rate in the middle and course in the bottom plot.\label{fig:Coursetraj}}
\end{figure}

Following this, we create a union set of the desired velocity trajectories as:
\begin{equation}\label{eq:desiredVelocities}
	\mathcal{U}_d = \{U_{d,1}(t), U_{d,2}(t), \ldots, U_{d,{N_U}}(t)\} \times \{ \chi_{d,1}(t), \chi_{d,2}(t), \ldots , \chi_{d,{N_\chi}}(t)\},
\end{equation}
resulting in a total of $N_U\cdot N_\chi$ desired velocity trajectories. Notice that the \gls{sog} trajectories in \eqref{eq:desiredVelocities} are continuously differentiable, while the course trajectories are twice continuously differentiable. Velocity trajectories containing non-feasible steady-state vessel velocities are removed from \eqref{eq:desiredVelocities} by checking the feasibility using the vessel model \eqref{eq:Model} together with the actuator saturation constraints.

Based on the desired velocity trajectories, we calculate the feedback-corrected position trajectories. To do this, we first predict the resulting \gls{sog} and course trajectories, $\bar U_i(t)$, $i\in [1,N_U]$ and $\bar \chi_i(t)$, $i\in[1,N_\chi]$, respectively, by simulating the closed-loop error dynamics of the vessel. In this article, we use a linear first order error model:
\begin{equation}\label{eq:errorModel}
  	\begin{aligned}
    	\dot{\tilde U} &= \frac{1}{T_{\tilde U}} \tilde U \\
    	\dot{\tilde \chi} &= \frac{1}{T_{\tilde \chi}} \tilde \chi,
  	\end{aligned}
\end{equation}
where $\tilde U = \bar U - U_d$, $\tilde \chi = \bar \chi - \chi_d$, and $T_{\tilde U}$ and $T_{\tilde \chi}$ are time constants. Using the error model \eqref{eq:errorModel}, the predicted \gls{sog} and course trajectories are found as:
\begin{equation}\label{eq:velocityPrediction}
  	\begin{aligned}
    	\bar U_i(t) &=  \tilde U_0 \mathrm{e}^{-\frac{1}{T_{\tilde U}}(t - t_0) } + U_{d,i}(t), & i \in [1,N_U],\\
    	\bar r_i(t) &=  \tilde r_0 \mathrm{e}^{-\frac{1}{T_{\tilde r}}(t - t_0) } + r_{d,i}(t), & i \in [1,N_\chi],
  	\end{aligned}
\end{equation}
where $\tilde U_0= U_0 - U_{d,0}$ and $\tilde \chi_0 = \chi_0- \chi_{d,0}$ introduces feedback in the prediction through the current \gls{sog} and course, $U_0$ and $\chi_0$, respectively. Similarly as \eqref{eq:desiredVelocities}, we construct a set of predicted velocity trajectories:
\begin{equation}\label{eq:predictedVelocities}
	\bar{\mathcal{U}} = \{\bar U_1(t), \bar U_2(t), \ldots, \bar U_{N_U}(t)\} \times \{ \bar \chi_1(t), \bar \chi_2(t), \ldots , \bar \chi_{N_\chi}(t)\}. 	
\end{equation}
Combinations of \gls{sog} and course trajectories that was considered infeasible when forming $\mathcal{U}_d$ are also removed from $\bar{\mathcal{U}}$. Following this, vessel position trajectories $\bar{\bs p}(t) = \begin{bmatrix} \bar N(t) & \bar E(t) \end{bmatrix}^T$ are calculated from the predicted velocity trajectories using a kinematic model:
\begin{equation}
  	\begin{aligned}
    	\dot{\bar{\bs p}} &= \begin{bmatrix} \cos(\bar\chi) \\ \sin(\bar\chi) \end{bmatrix} \bar U,
  	\end{aligned}
\end{equation}
which is simulated using the modified Euler method using the current position as the initial position. The predicted vessel position trajectories are combined in a set as:
\begin{equation}\label{eq:predictedPosition}
	\bar{\mathcal{P}} = \left\{\bar p(t; \bar U(t)) \big | (\bar U(t), \bar \chi(t)) \in \bar{\mathcal{U}} \right\}.
\end{equation}

To summarize, a single step of a trajectory is defined by the set of desired velocity trajectories $\mathcal{U}_d$, the set of predicted velocity trajectories $\bar{\mathcal{U}}$ and the set of set of predicted position trajectory $\bar{\mathcal{P}}$. A single-step of the trajectory generations is described in \Cref{alg:singleStepTraj}.
\begin{algorithm}
\caption{\label{alg:singleStepTraj}Single-step trajectory generation}
\begin{algorithmic}[1]
\Function{$traj\_step$}{$\bs \eta_0$, $\bs X_0$, $\bs \tau_0$, $\bs u_{d_0}$, $\dot U'_d$, $\dot r'_d$, $T$, $T_{ramp}$, $T_U$, $T_\chi$, $N_U$, $N_\chi$} 
	\State $\dot{\bs X}_{\min}, \dot{\bs X}_{\min} \gets$ possible acceleration using \eqref{eq:possibleAcc} and \eqref{eq:possibleActuator}.
	\State Construct $\dot {\bs U}_{samples}$ and $\dot {\bs r}_{samples}$ by sampling $A_d$ uniformly in SOG and course.
	\If{$\dot U'_d \in A_d$}
		\State $\dot U_{\max,i} = \dot U'_d$ for $i$ such that $\norm{\dot U_{\max,i} - \dot U'_d} = \underset{\dot U_{\max} \in {\bs U}_{samples}}{\min}\norm{\dot U_{\max} - \dot U'_d}$.
	\EndIf
	\If{$\dot r'_d \in A_d$}
		\State $\dot r_{\max,i} = \dot r'_d$ for $i$ such that $\norm{\dot r_{\max,i} - \dot r'_d} = \underset{\dot r_{\max} \in {\bs r}_{samples}}{\min}\norm{\dot r_{\max} - \dot r'_d}$.
	\EndIf
	\State $\dot U_{d,i}(t), U_{d,i}(t), i\in[1,N_U] \gets$ SOG trajectories using \eqref{eq:sog_acc} and \eqref{eq:velocity_trajs}.
	\State $\dot r_{d,i}(t), r_{d,i}(t), \chi_{d,i}(t), i\in[1,N_\chi] \gets$ course trajectories using \eqref{eq:course_acc} and \eqref{eq:velocity_trajs}.
	\State Form the set of desired velocities trajectories $\mathcal{U}_d$ using \eqref{eq:desiredVelocities}. Remove infeasible trajectories.
	\State Form the set of predicted velocities trajectories $\bar{\mathcal{U}}$ using \eqref{eq:velocityPrediction} and \eqref{eq:predictedVelocities}.
	\State Form the set of predicted position trajectories $\bar{\mathcal{P}}$ using \eqref{eq:predictedPosition}.
	\State \Return $\mathcal{U}_d$, $\bar{\mathcal{U}}$ and $\bar{\mathcal{P}}$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{Trajectory generation: The full trajectory generation}
A full trajectory consists of multiple maneuvers, where each is considered as a sub-trajectory and constructed using the single-step procedure. This naturally forms a tree structure, which is initialized with the initial state as the root node. The single step procedure is then performed on the root node, generating a number of sub-trajectories as leaf nodes. Following this, the the single-step procedure is performed on each of the leaf nodes, adding the next sub-trajectory to the trajectories and expanding the tree. This procedure is then repeated until the desired number of branches is constructed. Using the same number of \gls{sog} and course maneuvers in each step would result in the tree growing exponentially with the number of branches. To limit the growth to a feasible level we therefore allow for choosing a different number of \gls{sog} and course maneuvers at each branch, for instance keeping the \gls{sog} constant in all steps except the first, only allowing the \gls{sog} to be changed during the first maneuver.

The remaining parameters for each step can also be chosen differently, and in principle the acceleration trajectories could also be designed using a different structure. However, we choose to use the same acceleration trajectory structure for each step, while also keeping the ramp time and maneuver time lengths constant. This leaves only the step time length and number of \gls{sog} and course maneuvers as parameters that change during the steps. Choosing different step time lengths can be considered as an \gls{mpc} input blocking scheme, requiring that the step lengths are integer dividable by the algorithm sample time. To execute a full maneuver, the algorithm sample time is required to be equal to the first step length, requiring consecutive step lengths to be integer dividable by the first step length.

A full trajectory generation can hence be defined by the following parameters:
\begin{itemize}
  	\item An initial vessel state including the current desired velocity.
  	\item The number of branches, defined as $B$.
  	\item The prediction time of each step $\bs T = \begin{bmatrix} T_0 & T_1 & \ldots & T_{B} \end{bmatrix}$, the ramp time $T_{ramp}$ and the \gls{sog} and course maneuver lengths $T_U$ and $T_\chi$, respectively.
  	\item The number of \gls{sog} maneuvers in each step $\bs N_U = \begin{bmatrix} N_{U_0} & N_{U_1} & \ldots & N_{U_B} \end{bmatrix}$.
  	\item The number of course maneuvers in each step $\bs N_\chi = \begin{bmatrix} N_{\chi_0} & N_{\chi_1} & \ldots & N_{\chi_B} \end{bmatrix}$.
\end{itemize}

The trajectory generation is described in \Cref{alg:fullTraj}. A set of predicted vessel trajectories with $\bs T = \begin{bmatrix} 5~\si{\second} & 10~\si{\second} & 10~\si{\second} \end{bmatrix}$ is shown in \Cref{fig:postraj}. The trajectories are $25~\si{\second}$ long in total, and have $5$ course candidates at the first step and three in the later branches, while there for illustrational purposes are only one \gls{sog} candidate at each step. Hence, $\bs N_U = \begin{bmatrix} 1 & 1 & 1 \end{bmatrix}$ and $\bs N_r = \begin{bmatrix} 5 & 3 & 3 \end{bmatrix}$. The ramp time and maneuver lengths are chosen as $T_{ramp} = 5~\si{\second}$ and $T_U = T_\chi = 5~\si{\second}$, respectively.

\begin{figure}
	\centering
	\includegraphics[width=.8\textwidth]{figures/traj.pdf}
  	%\includegraphics[width=.7\textwidth]{figures/HDWPosTraj.png}
  	\caption{Position trajectories\label{fig:postraj}}
\end{figure}

\begin{algorithm}
\caption{\label{alg:fullTraj}Full trajectory generation}
\begin{algorithmic}[1]
\Function{$full\_traj$}{$\bs \eta_0$, $\bs X_0$, $\bs u_{d_0}$, $T$, $T_{ramp}$, $T_U$, $T_\chi$, $N_U$, $N_r$} 
	\State Initialize trajectory tree $\mathcal{T} = \emptyset$
	\State Set constant parameters $T_{ramp}, T_U, T_\chi$
	\State Set level-dependent parameters $\bs T, \bs N_U, \bs N_\chi$
	\State $\mathcal{T}.add\_node\left(level = 0, \bs \eta_0, \bs X_0, \bs u_{d_0}\right)$ \Comment{Add root node}
	\For{$l = 1:length(\bs T)$} \Comment{Loop through all levels}
		\If{$l = 1$} \Comment{First step}
			\State $T^{1} \gets \bs T[1]$
			\State $N_U^{1} \gets \bs N_U[1]$
			\State $N_\chi^{1} \gets \bs N_\chi[1]$
			\State $(\bs \eta_0^{1}, \bs X_0^{1}, \bs u_{d_0}^{1}) \gets \mathcal{T}.get\_root\_node()$
			\State $\bs \tau_0^{1} \gets inverse\_vessel\_model\left(\bs X_0^{1}\right)$
			\State $(\dot U'_d, \dot r'_d) \gets desired\_acceleration()$ \Comment{Calculate desired acceleration}
			\State $(\mathcal{U}_d^{1}, \bar{\mathcal{U}}^{1}, \bar{\mathcal{P}}^{1}) = traj\_step\left(\bs \eta_0^{1}, \bs X_0^{1}, \bs \tau_0^{1}, \bs u_{d_0}^{1}, \dot U'_d, \dot r'_d, T^{1}, T_{ramp}, T_U, T_\chi, N_U^{1}, N_\chi^{1}\right)$
			\ForAll{$(\bar{\bs p}(t), \bar{\chi}(t), \bar{U}(t), \bs u_{d}(t)) \in (\bar{\mathcal{P}^{1}}, \bar{\mathcal{U}^{1}}, \mathcal{U}_d^{1})$} 
				\State $\bar{\bs X}(t) \gets \left[\bar{U}(t), \dot{\bar{\chi}}(t)\right]$ \Comment{Form predicted vessel velocity vector} 
				\State $\bar{\bs \eta}(t) \gets \left[\bar{\bs p}(t), \bar{\chi}(t)\right]$ \Comment{Form predicted vessel pose vector} 
				\State $\mathcal{T}.add\_node\left(level = 1, \bar{\bs \eta}(end), \bar{\bs X}(end), \bs u_{d}(end)\right)$ \Comment{Add new node at level 1}
				\State $\mathcal{T}.add\_edge\left(from = root, \bar{\bs \eta}(t), \bar{\bs X}(t), \bs u_{d}(t)\right)$ \Comment{Add edge to the new node}
			\EndFor
		\Else
			\State $T^{l} \gets \bs T[l]$
			\State $N_U^{l} \gets \bs N_U[l]$
			\State $N_\chi^{l} \gets \bs N_\chi[l]$
			\For{$n = 1:\mathcal{T}.num\_nodes(level = l-1)$}
				\State $(\bar{\bs \eta}_0^{l,n}, \bar{\bs X}_0^{l,n}, \bs u_{d_0}^{l,n}) \gets \mathcal{T}.get\_node(level = l-1, node = n)$
				\State $\bar{\bs \tau}_0^{l,n} \gets inverse\_vessel\_model\left(\bar{\bs X}_0^{l,n}\right)$
				\State $(\dot U'_d, \dot r'_d) \gets desired\_acceleration()$ \Comment{Calculate desired acceleration}
				\If{$N_U$ = 1}
					\State $\dot U'_d \gets 0$ \Comment{Constant SOG}
				\EndIf
				\State $(\mathcal{U}_d^{l,n}, \bar{\mathcal{U}}^{l,n}, \bar{\mathcal{P}}^{l,n}) = traj\_step\left(\bar{\bs \eta}_0^{l,n}, \bar{\bs X}_0^{l,n}, \bar{\bs \tau}_0^{l,n}, \bs u_{d_0}^{l,n}, \dot U'_d, \dot r'_d, T^{l}, T_{ramp}, T_U, T_\chi, N_U^{l}, N_\chi^{l}\right)$
				\ForAll{$(\bar{\bs p}(t), \bar{\chi}(t), \bar{U}(t), \bs u_{d}(t)) \in (\bar{\mathcal{P}^{l,n}}, \bar{\mathcal{U}^{l,n}}, \mathcal{U}_d^{l,n})$} 
					\State $\bar{\bs X}(t) \gets \left[\bar{U}(t), \dot{\bar{\chi}}(t)\right]$ \Comment{Form predicted vessel velocity vector} 
					\State $\bar{\bs \eta}(t) \gets \left[\bar{\bs p}(t), \bar{\chi}(t)\right]$ \Comment{Form predicted vessel pose vector} 
					\State $\mathcal{T}.add\_node\left(level = l, \bar{\bs \eta}(end), \bar{\bs X}(end), \bs u_{d}(end)\right)$ \Comment{Add new node at level $l$}
					\State $\mathcal{T}.add\_edge\left(from=(l-1,n), \bar{\bs \eta}(t), \bar{\bs X}(t), \bs u_{d}(t)\right)$ \Comment{Add edge to the new node}
				\EndFor
			\EndFor
		\EndIf
	\EndFor
	\State $\mathcal{H} \gets \emptyset$
	\State $\mathcal{U}_d \gets \emptyset$
	\For{$n = 1:\mathcal{T}.num\_nodes(level = end)$} \Comment{Loop through all nodes of the last level}
		\State $(\bar{\bs \eta}_n(t), \bs u_{d,n}(t)) \gets \mathcal{T}.backtrace\_path(from = (end, n), to = root\_node)$
		\State $\mathcal{H} \gets \mathcal{H} \cup \{\bar{\bs \eta}_n(t)\}$
		\State $\mathcal{U}_d \gets \mathcal{U}_d \cup \{\bs u_{d,n}(t)\}$
	\EndFor
	\State \Return $(\mathcal{H}, \mathcal{U}_d)$
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{Calculating a desired acceleration}
In each step of the trajectory generation, a desired acceleration $(\dot U_d', \dot r_d')$ can be used to include a desired maneuver in the search space. We therefore use a guidance algorithm to ensure that there exists a candidate maneuver in the search space which will converge to the desired trajectory inputted to the \gls{bc-mpc} algorithm. To achieve this, we use a modified version of a path tracking algorithm presented in~\cite{Breivik2004}. In this article, the authors present a control law to ensure vessel convergence to a curved path. The control law is based on \gls{los} guidance~\cite{Fossen2011}, together with defining a desired point on the path which the velocity of is controlled, named the path particle (PP). The desired course is stated as:
\begin{equation}
	\chi_{d,LOS} = \chi_t + \arctan\left(- \frac{e}{\Delta}\right),
\end{equation}
where $\chi_t$ is the path angle at the desired point, $e$ is the cross-track error and $\Delta > 0$ is the lookahead distance. The path particle velocity along the path is stated as:
\begin{equation}\label{eq:trackingUpp}
	U_{PP} = U \cos(\chi - \chi_t) + \gamma s,
\end{equation}
where $U$ is the vessel speed, $\gamma > 0$ is a tuning parameter and $s$ is the along-track distance. This control law controls the velocity along the path $U_{PP}$ as a function of the vessel speed, course and the along-track distance to the path particle, letting the vessel converge towards the path with a constant speed. We rather want to be able to follow a desired trajectory, by controlling the vessel speed and course based on the desired trajectory. We therefore fix the path particle at the desired position on the trajectory, given the current time, and by reformulating \eqref{eq:trackingUpp} we obtain a desired vessel speed given a fixed along-path velocity:
\begin{equation}
	U_{d,LOS} = \begin{cases}	\frac{U_{t} - \gamma s}{\cos(\chi - \chi_t)}  & \text{if } \lvert \cos(\chi - \chi_t) \rvert > \epsilon \\
						\frac{U_{pp} - \gamma s}{\epsilon}  & \text{else,} \end{cases}
\end{equation}
where $U_t$ is the desired trajectory velocity and $\epsilon > 0$ is a small constant to avoid division by zero. Given a desired speed and course, we compute the desired \gls{sog} and course acceleration:
\begin{equation}
	\begin{aligned}
		\dot U_d' &= \frac{U_{d,LOS} - U_{d,0}}{T_U - T_{ramp}} \\
		\dot r_d' &= \frac{\chi_{d,LOS} - \chi_{d,0}}{T_{ramp}\left(T_\chi - 2 T_{ramp}\right)},
	\end{aligned}
\end{equation}
which can be found by solving \eqref{eq:velocity_trajs} for the final desired \gls{sog} and course. Notice that in cases where there is only one \gls{sog} and/or course maneuver, the corresponding desired acceleration should be selected as zero to keep a constant speed and/or course.

\subsection{Selecting the optimal trajectory}
Given the set of possible trajectories, we solve an optimization problem to select the optimal trajectory with the set of trajectories forming the search space. We start by defining a cost function to assign a cost to each trajectory:
\begin{equation}\label{eq:objFunc}
 	G(\bar{\bs \eta}(t), \bs u_d(t)) = w_{\text{al}}\text{align}(\bar{\bs \eta}(t); \bs p_d(t)) + w_{\text{av}}\text{avoid}(\bar{\bs \eta}(t)) + w_{\text{h}}\text{hyst}(\bs u_d(t)),
\end{equation} 
where $(\bar{\bs \eta}(t), \bs u_d(t))$ is the predicted vessel position and desired velocity of a candidate trajectory, $\text{align}(\bar{\bs \eta}(t); \bs p_d(t))$ measures the alignment between the predicted position trajectory and a desired trajectory $\bs p_d(t)$, $\text{avoid}(\bar{\bs \eta}(t))$ assigns cost to trajectories traversing close to obstacles while $\text{hyst}(\bs u(t))$ introduces hysteresis in the objective function to avoid wobbly behavior. The parameters $w_{\text{al}}, w_{\text{av}}, w_{\text{h}} \geq 0$ are tuning parameters to control the weighting of the different objective terms. Using \eqref{eq:objFunc}, we define the optimization problem:
\begin{equation}\label{eq:ocp}
	\bs u_d(t) = \underset{(\bar{\bs \eta}_k(t), \bs u_{d,k}(t)) \in (\mathcal{H}, \mathcal{U}_d)}{\text{argmin}} G(\bar{\bs \eta}_k(t), \bs u_{d,k}(t)).
\end{equation}
\todo[inline]{$\mathcal{H}$ er ikke brukt tidligere i teksten, bare i pseudokoden. $\bar{\mathcal{P}}$ er brukt for position trajectory, men ikke med heading/kurs.}

The next sections describe the different terms of the objective function \eqref{eq:objFunc}.

\subsection{Trajectory alignment}
The alignment between the desired trajectory and a candidate trajectory is used in the objective function \eqref{eq:objFunc} to motivate the algorithm to follow the desired trajectory. Given a desired path $\bs p_d(t) : \mathrm{R}^+ \to \mathrm{R}^2$, required to be $C^1$, we obtain a desired course as
\begin{equation}
  	\chi_d(t) = \text{atan2}(\dot E_d(t), \dot N_d(t)),
\end{equation}
where $\bs p_d = \begin{bmatrix} N_d & E_d \end{bmatrix}^T$. Given this, we define a weighted metric of euclidean distance and orientation error as
\begin{equation}
  	\text{align}(\bar{\bs \eta}(t); \bs p_d(t)) = \sum_{t = t_1}^{t_N} w_p\norm{\begin{bmatrix} \bar N(t) \\ \bar E(t) \end{bmatrix} - \bs p_d(t)}_2 + w_\chi |\Upsilon\left(\bar\chi(t) - \chi_d(t)\right)|,
\end{equation}\todo{Er tid riktig angitt her? $t_1$->$t_N$?}
where $w_p$ and $w_\chi > 0$ are weights controlling the influence of the Euclidean and angular error, respectively, while $\Upsilon: \mathbb{R} \to S^1$ maps an angle to the domain $[-\pi,\pi)$. For simplicity, we fix $w_p = 1$ and leave $w_\chi$ to control the weighting.

\subsection{Obstacle avoidance}
Obstacle avoidance is achieved by penalizing predicted vessel position trajectories with small distances to obstacles. Furthermore, we define three regions around the obstacles named the collision, safety and margin regions, respectively. The idea behind this is to make it possible use different gradients on the penalty depending on how close the ownship is to the obstacle, which should improve the robustness with respect to noise on the obstacle estimates.

We define a time-varying vector between obstacle $i$ and a predicted vessel trajectory as:
\begin{equation}\label{eq:obstacleVector}
   	\bs r_i(\bar{\bs \eta}(t); \bs p_i(t)) = \bs p_i(t) - \begin{bmatrix} \bar N(t) \\ \bar E(t) \end{bmatrix},
\end{equation}
where $\bs r_i = \begin{bmatrix} r_{N,i} & r_{E,i} \end{bmatrix}^T$ and $\bs p_i(t)$ is the position of obstacle $i$ at time $t$. The obstacle position in future time is computed under the common assumption that an obstacle will keep the current speed and course~\cite{Johansen2016,Kuwata2014,Eriksen2018}, which is a reasonable assumption for relatively short time periods. More complex techniques can also be applied for predicting the future position of obstacles, for instance based on historic \gls{ais} data~\cite{Hexeberg2017} or by estimating the turn rate of the obstacles~\cite{Flaaten2017}. Using \eqref{eq:obstacleVector}, we define the distance and relative bearing to obstacle $i$ given a predicted vessel trajectory $\bar{\bs \eta}(t)$ as:
\begin{equation}
  	\begin{aligned}
    	d_i(\bar{\bs \eta}(t)) &= \norm{\bs r_i(\bar{\bs \eta}(t))}_2^2 \\
    	\beta_i(\bar{\bs \eta}(t);\bs p_i(t)) &= \Upsilon\left(\text{atan2}\big(r_{E,i}(\bar{\bs \eta}(t)), r_{N,i}(\bar{\bs \eta}(t))\big) - \chi_i(t)\right),
  	\end{aligned}
\end{equation}
where $\chi_i(t)$ is the course of obstacle $i$, calculated as $\chi_i(t) = \text{atan2}\left(\dot E_i, \dot N_i \right)$ with $\bs p_i(t) = \begin{bmatrix} N_i & E_i \end{bmatrix}^T$. The distance $d_i$ and relative bearing $\beta_i$ is illustrated in \Cref{fig:obsDistPose}. It should be noted that given the relative bearing, the avoidance functions may be designed to produce \gls{colregs}-aware maneuvers.\todo{fjerne?}
\begin{figure}
  	\centering
  	\includegraphics[width=.5\textwidth]{figures/obsDistPose.pdf}
  	\caption{\label{fig:obsDistPose}Distance $d_i$ and relative bearing $\beta_i$ to obstacle $i$. The ownship is marked O/S.}
\end{figure}

The obstacle distance and relative bearing is used to calculate a penalty function, which we use to define the avoidance function as
\begin{equation}
  	\text{avoid}(\bar{\bs \eta}(t)) = \sum_{i=1}^M \sum_{t=t_1}^{t_N} w_{i,t} \text{penalty}_i(\bar{\bs \eta}(t)),
\end{equation}
where $\text{penalty}_i(\bar{\bs \eta}(t))$ assigns a penalty to the predicted vessel trajectory $\bar{\bs \eta}(t)$ at time $t$ with respect to obstacle $i$, while $w_{i,t}$ are time and obstacle dependent weights. The penalty function will be further discussed in the following subsections.

\subsubsection{Circular penalty}
When using a circular penalty, the relative bearing to the obstacle does not matter. A circular penalty function can be defined as:

where:
\begin{equation}\label{eq:circularPenaltyEq}
  	\text{penalty}_{i, \text{circular}}(\bar{\bs \eta}(t)) = 
  	\begin{cases}
  	  	1    & \text{if } d_i < D_0 \\
  	  	1 + \frac{\gamma_1 - 1}{D_1 - D_0} (d_i - D_0)    & \text{if } D_0 \leq d_i < D_1 \\
  	  	\gamma_1 - \frac{\gamma_1}{D_2 - D_1} (d_i - D_1)    & \text{if } D_1 \leq d_i < D_2 \\
  	  	0       & \text{else},
  	\end{cases}
\end{equation}
where the parameters of $d_i(\bar{\bs \eta}(t))$ are omitted for notational simplicity. The variables $D_2 > D_1 > D_0 > 0$ are the margin, safety and collision region sizes, respectively, while $\gamma_1 \in (0,1)$ is a tuning parameter controlling the cost gradient inside the margin and safety regions. The function is illustrated in \Cref{fig:CicPenalty}.
\begin{figure}
  	\centering
  	\begin{subfigure}[b]{.48\textwidth}
  	  	\includegraphics[width=\textwidth]{figures/circularObsCostFunc.pdf}
  	  	\caption{\label{fig:circularObsCostFunc}Function value.}
  	\end{subfigure}\quad
\begin{subfigure}[b]{.48\textwidth}
  	  	\includegraphics[width=\textwidth]{figures/circularObsCost.pdf}
  	  	\caption{\label{fig:circularObsCostRegions}Function regions. The red region is the collision region, yellow is the safety region and green is the margin region.}
  	\end{subfigure}
  	\caption{\label{fig:CicPenalty}Circular penalty function.}
\end{figure}

\subsubsection{Elliptical penalty}
The motivation behind an an elliptical penalty function is that it is considered more dangerous to be located in front of an obstacle than on the side or behind. This allows the ownship to travel closer to an obstacle if passing on the side than passing in front, which is intuitive. In addition, passing behind the vessel should also be considered less dangerous than passing in front. The elliptic penalty is designed similarly as the circular penalty~\eqref{eq:circularPenaltyEq}, but allowing the sizes of the obstacle regions $D_0, D_1$ and $D_2$ to be dependent on the relative bearing $\beta_i$. An ellipse is defined in polar coordinates as:
\begin{equation}
  	r(\theta )={\frac {ab}{\sqrt {(b\cos \theta )^{2}+(a\sin \theta )^{2}}}},
\end{equation}\todo{fjerne ellipseligninga?}
where $a$ and $b$ are the lengths of the major and minor axis, respectively. Using this, we define the function regions as:
\begin{equation}\label{eq:elliptical_regions}
  	D_k(\beta_i) = \begin{cases}
     	\frac{a_k b_k}{\sqrt{(b_k \cos \beta_i )^{2}+(a_k\sin \beta_i )^{2}}} & \text{if } |\beta_i| < \frac{\pi}{2} \\
     	b_k & \text{else},
  	\end{cases}
\end{equation}
where $k\in\{0,1,2\}$, while $a_k$ and $b_k$ are major and minor axis sizes as illustrated in \Cref{fig:ellipticalObsCostRegions}. The parameters of $\beta_i(\bar{\bs \eta}(t))$ are omitted for notational simplicity. Using this function results in a elliptical penalty function in front of the vessel, and a circular penalty function behind the vessel, as shown in \Cref{fig:ellipticalObsCostRegions}.
\begin{figure}
  	\centering
  	\includegraphics[width=0.48\textwidth]{figures/ellipticalObsCost.pdf}
  	\caption{\label{fig:ellipticalObsCostRegions}Elliptical function regions.}
\end{figure}

\subsubsection{Elliptical COLREGs penalty}
As mentioned, the relative bearing can be utilized to produce \gls{colregs}-aware maneuvers\todo{husk å fjerne sammen med setningen om COLREGs-aware tidligere i tilfelle}. In order to ensure compliance with the case of the give-way vessel failing in its duty to avoid collision (rule $17$), it is not beneficial to constrain the algorithm to strictly follow the overtaking, head-on and crossing rules ($13-15$), as maneuvers violating these rules may be required to fulfill rule $17$. However, the vessel should choose maneuvers compliant with rules $13-15$ when this is possible. We therefore suggest an alternative penalty function to motivate the algorithm to choose \gls{colregs}-aware maneuvers simply by extending the function regions on the starboard side of obstacles. The regions are defined using three ellipses and one circle as:
\begin{equation}\label{eq:COLREGs_regions}
  	D_k(\beta_i) = \begin{cases}
     	b_k & \text{if } \beta_i < -\frac{\pi}{2} \\
     	\frac{a_k b_k}{\sqrt{(b_k \cos \beta_i )^{2}+(a_k\sin \beta_i )^{2}}} & \text{if } -\frac{\pi}{2} \leq |\beta_i| < 0 \\
     	\frac{a_k c_k}{\sqrt{(c_k \cos \beta_i )^{2}+(a_k\sin \beta_i )^{2}}} & \text{if } 0 \leq |\beta_i| < \frac{\pi}{2} \\
     	\frac{b_k c_k}{\sqrt{(c_k \cos \beta_i )^{2}+(b_k\sin \beta_i )^{2}}} & \text{if } \frac{\pi}{2} \leq |\beta_i|,
  	\end{cases}
\end{equation}
where $c_k = b_k + d_{\text{COLREGs}}$, with $d_{\text{COLREGs}}$ controlling the region expansion of the starboard side of the obstacle.

The regions are illustrated in \Cref{fig:ellipticalColregsObsCostRegions}.
\begin{figure}
  	\centering
  	\includegraphics[width=0.54\textwidth]{figures/ellipticalCOLREGSObsCost.pdf}
  	\caption{\label{fig:ellipticalColregsObsCostRegions}Elliptical COLREGs function regions.}
\end{figure} 
If we were to use \eqref{eq:circularPenaltyEq} with $D_k$ from \eqref{eq:COLREGs_regions} as the penalty function, the entire collision region would have a constant penalty. This poses a potential problem since all points inside the region is considered to be equally costly. For the non-\gls{colregs} elliptical regions, this regions is so small that the impact will be quite low. For the elliptical \gls{colregs} penalty function, it is, however, natural to have a non-constant cost inside the collision region since this is rather large. We therefore define the elliptical \gls{colregs} penalty function as:
\begin{equation}\label{eq:ellipticalColregsPenaltyEq}
  	\text{penalty}_{i, \text{COLREGs}}(\bar{\bs \eta}(t)) = \text{inner\_penalty}_i(\bar{\bs \eta}(t)) + 
  	\begin{cases}
  	  	1    & \text{if } d_i < D_0 \\
  	  	1 + \frac{\gamma_1 - 1}{D_1 - D_0} (d_i - D_0)    & \text{if } D_0 \leq d_i < D_1 \\
  	  	\gamma_1 - \frac{\gamma_1}{D_2 - D_1} (d_i - D_1)    & \text{if } D_1 \leq d_i < D_2 \\
  	  	0       & \text{else},
  	\end{cases}
\end{equation}
where $D_k$ is given by \eqref{eq:COLREGs_regions} and
\begin{equation}
	\text{inner\_penalty}_i(\bar{\bs \eta}(t)) = 
	\begin{cases}
  	  	1    & \text{if } d_i < D_{0}^* \\
  	  	1 - \frac{y_b(d_i, \beta_i)}{d_{\text{COLREGs}}}    & \text{if } D_{0}^* \leq d_i < D_0,
  	\end{cases}
\end{equation}
where $D_{0}^*$ is given as $D_0$ in \eqref{eq:elliptical_regions} and $y_b(d_i, \beta_i)$ is the distance from the $D_{0}^*$ region the point $(d_i, \beta_i)$ in the y-direction of the obstacle body frame. This is illustrated in \Cref{fig:ellipticalColregsDistFromDinner}.
\begin{figure}
  	\centering
  	\includegraphics[width=0.3\textwidth]{figures/ellipticalCOLREGSDistFromDinner.pdf}
  	\caption{\label{fig:ellipticalColregsDistFromDinner}Variables for the inner penalty function for the elliptical COLREGs penalty function given a point $(d_i, \beta_i)$.}
\end{figure}
\todo[inline]{Fjerne de vi ikke bruker her, skrive sammen i ett kapittel så vi kan restrukturere til to subkapitler i kapittel 3.}

\subsubsection{Avoidance weights}
The weights $w_{i,t}$ can be useful for prioritizing vessels in multi-encounter situations while also facilitating time-dependent weighting for instance as a heuristic measure of uncertainty.

Prioritizing vessels in multi-encounter situations can be done based on properties of the vessel (for instance vessel type, size, speed, etc.) which can differentiate the importance of avoiding the given obstacles in severe situations.

Estimates of obstacle trajectories are subject to uncertainties. A simple heuristic way to incorporate such uncertainty in the optimization is to use time-dependent weights scaled with the uncertainty. In this case, the size of the obstacle regions should also be scaled with the uncertainty.

For simplicity, we keep the weights constant at $w_{i,t} = 1 \, \forall \,i,t$.

\subsection{Hysteresis cost}
To increase the robustness to noise and fluctuations in the obstacle estimates, we introduce hysteresis in the objective function. This will also increase the robustness to noise in the vessel state estimates and external disturbances, for instance wave induced motion.

Denoting the desired velocity trajectory from the previous iteration as $\bs u_d^-(t)$, the hysteresis cost is computed as:
\begin{equation}
  \text{hyst}(\bs u_d(t)) = \begin{cases}1 & \text{if } \sum_{t = t_1}^{t_{N_1}} \left|U_d(t) - U_d^-(t)\right| > e_{U,\min} \text{ or } \sum_{t = t_1}^{t_{N_1}} \left|\chi_d(t) - \chi_d^-(t)\right| > e_{\chi,\min}\\ 0 & \text{else},\end{cases}
\end{equation}
where $\bs u_d(t) = \begin{bmatrix} U_d(t) & \chi_d(t) \end{bmatrix}^T$, and $t_1, t_2, \ldots t_{N_1}$\todo{sjekk tid} are the time steps of the first maneuver of the desired vessel trajectory $\bs u_d(t)$, with $t_{N_1}=T_0$. The variables $e_{U,\min}$ and $e_{\chi,\min}$ denote the minimum difference between the previous desired velocity trajectory and the candidates, defined as:
\begin{equation}
  \begin{aligned}
    e_{U,\min} &= \underset{\bs u_d(t) \in \mathcal{U}_d}{\text{min}} \sum_{t = t_1}^{t_{N_1}} \norm{U_d(t) - U_d^-(t)} \\
    e_{\chi,\min} &= \underset{\bs u_d(t) \in \mathcal{U}_d}{\text{min}} \sum_{t = t_1}^{t_{N_1}} \norm{\chi_d(t) - \chi_d^-(t)},
  \end{aligned}
\end{equation}
with $\bs u_d^-(t) = \begin{bmatrix} U_d^-(t) & \chi_d^-(t) \end{bmatrix}^T$. The hysteresis term is zero if the first sub-trajectory of the candidate desired velocity trajectory is the one closest to the desired velocity trajectory from the previous iteration.

\todo[inline]{Litt sub-optimal kapittelinndeling her. Ideelt sett burde 3.3-3.5 vært subkapitler av 3.2.}
% \subsection{Algorithm overview}
% The \gls{bc-mpc} algorithm architecture is shown in \cref{fig:bc-mpc_architecture}. The algorithm inputs a desired trajectory, which can originate from either another \gls{colav} algorithm or directly from a user. The guidance function receives the desired trajectory, and computes a desired acceleration given a vessel state and time specified by the trajectory generation. The trajectory generation block creates a set of possible vessel trajectories, given an initial vessel state, initial desired velocity and desired accelerations from the guidance function. Notice that this is where feedback enters the algorithm. A tracking system provides obstacle estimates, which are used to calculate the obstacle avoidance cost for each possible velocity trajectory. The optimization block computes the optimal velocity trajectory based on the objective function \eqref{eq:objFunc}, and outputs this as the desired velocity trajectory to the vessel controller \eqref{eq:vesselController}.
% \begin{figure}
% 	\centering
% 	\includegraphics[width=\textwidth]{figures/bc-mpc_architecture.pdf}
% 	\caption{\label{fig:bc-mpc_architecture}BC-MPC algorithm overview.}
% \end{figure}\todo[inline]{\cref{fig:bc-mpc_architecture} can be more detailed with blocks inside the optimization ("hysteresis", avoidance, align) showing the architecture more explicitly. One can also show more explicitly where COLREGs awareness is included.}
